Implicit Bias of Gradient Descent on Reparametrized Models: On Equivalence to Mirror Descent

As part of the effort to understand implicit bias of gradient descent in overparametrized models, several results have shown how the training trajectory on the overparametrized model can be understood as mirror descent on a different objective. The main result here is a characterization of this phenomenon under a notion termed commuting parametrization, which encompasses all the previous results in this setting. It is shown that gradient flow with any commuting parametrization is equivalent to continuous mirror descent with a related Legendre function. Conversely, continuous mirror descent with any Legendre function can be viewed as gradient flow with a related commuting parametrization. The latter result relies upon Nash's embedding theorem.

==> sections/main_results__Zhiyuan_Li_s_conflicted_copy_2022-07-06_1_.tex <==
\section{Any gradient flow with commuting parametrization is a mirror flow}\label{sec:CGF_to_MF}

\subsection{Commuting parametrization}
We now formalize the notion of commuting parametrization.
We remark that $M$ is a smooth submanifold of $\RR^D$, and it is the domain of 
the parametrization $G$.

\begin{definition}[Commuting parametrization]\label{def:commuting_param}
Let $M$ be a smooth submanifold of $\RR^D$.
A $\mathcal{C}^2$ parametrization $G: M \to \RR^d$ is \emph{commuting} in a subset $S\subseteq M$ 
if and only if for any $i, j \in [d]$, the Lie bracket 
$[\nabla G_i, \nabla G_j](x) = 0$ for all $x \in S$. 
Moreover, we say $G$ is a \emph{commuting parametrization} if it is commuting in the 
entire $M$.
\end{definition}

In particular, when  $M$ is an open subset of $\RR^d$, $\{\nabla G_i\}_{i=1}^d$ 
are ordinary gradients in $\RR^D$, and the Lie bracket between 
any pair of $\nabla G_i$ and $\nabla G_j$ is given by 
\begin{align*} 
[\nabla G_i, \nabla G_j](x) = \nabla^2 G_j(x) \nabla G_i(x) - \nabla^2 G_i(x) \nabla G_j(x).
\end{align*}
This provides an easy way to check whether $G$ is commuting or not.

\begin{figure}[t]
\vspace{-1cm}
    \centering
    \tikzset{mycirc/.style={circle,fill=black,inner sep=0pt,minimum size=3pt}}
    \begin{tikzpicture}[scale=1.5]
    \draw[-{Latex[length=3mm,width=2mm]}](0, 0) -- (0, 1.57);
    \node (A) at (-0.4, 0.8) {{ $-\nabla G_i$}};
    \node (A) at (0.15, 0.8) {{ $t_i$}};
    \draw[-{Latex[length=3mm,width=2mm]}](0, 0) -- (3.17, 0);
    \node (A) at (1.6, -0.2) {{ $-\nabla G_j$}};
    \node (A) at (1.6, 0.15) {{ $t_j$}};
    \draw[-{Latex[length=3mm,width=2mm]}] (0, 1.6) -- (3.17, 1.6);
    \node (A) at (1.6, 1.75) {{ $-\nabla G_j$}};
    \node (A) at (1.6, 1.4) {{ $t_j$}};
    \draw[-{Latex[length=3mm,width=2mm]}] (3.2, 0) -- (3.2, 1.57);
    \node (A) at (3.6, 0.8) {{$-\nabla G_i$}};
    \node (A) at (3.05, 0.85) {{ $t_i$}};
    \filldraw[black] (0, 0) circle (1pt) node[anchor=north east]{$x$};
    \filldraw[black] (0, 1.6) circle (1pt) node[anchor=south east]{$\phi_{G_i}^{t_i}(x)$};
    \filldraw[black] (3.2, 0) circle (1pt) node[anchor=north west]{$\phi_{G_j}^{t_j}(x)$};
    \filldraw[black] (3.2, 1.6) circle (1pt) node[anchor=south west]{$\phi_{G_i}^{t_i}
        \circ \phi_{G_j}^{t_j}(x) = \phi_{G_j}^{t_j} \circ \phi_{G_i}^{t_i}(x)$};
    \end{tikzpicture}
    \caption{Illustration of commuting parametrizations.
    Suppose $G: M \to \RR^d$ is a commuting parametrization satisfying \Cref{assump:domain}, then starting from any $x \in M$, first moving along $-\nabla G_i$ for time $t_i$ then moving along $-\nabla G_j$ for time $t_j$ yields the same result as first moving along $-\nabla G_j$ for time $t_j$ then moving along $-\nabla G_i$ for time $t_i$ does, i.e., $\phi_{G_i}^{t_i} \circ \phi_{G_j}^{t_j}(x) = \phi_{G_j}^{t_j} \circ \phi_{G_i}^{t_i}(x)$.}
    \label{fig:commuting_vec_fields}
\end{figure}

The above definition of commuting parametrizations builds upon the differential 
properties of the gradient vector fields $\{\nabla G_i\}_{i=1}^d$, where 
each Lie bracket $[\nabla G_i, \nabla G_j]$ characterizes the change of 
$\nabla G_j$ along the flow generated by $\nabla G_i$.
In particular, when $G$ is a commuting parametrization satisfying \Cref{assump:domain}, 
it is further equivalent 
to a characterization of `commuting' in the integral form, as summarized in
\Cref{thm:commuting_equivalence}.
Also see \Cref{fig:commuting_vec_fields} for an illustration.


\begin{theorem}[Adapted from Theorem 9.44 in~\citet{lee2013smooth}]\label{thm:commuting_equivalence}
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a $\cC^2$
parametrization.
For any $i, j \in [d]$, $[\nabla G_i, \nabla G_j](x) = 0$ for all $x \in M$ if and only if for any $x \in M$,  whenever both $\phi_{G_i}^s \circ \phi_{G_j}^t(x)$ and $\phi_{G_j}^t \circ \phi_{G_i}^s(x)$ are well-defined for all $(s,t)$ in some rectangle $\cI_1 \times \cI_2$ where $\cI_1, \cI_2 \subseteq \RR$ are open intervals, it holds that $\phi_{G_i}^s \circ \phi_{G_j}^t(x) = \phi_{G_j}^t \circ \phi_{G_i}^s(x)$ for all $(s,t)\in \cI_1 \times \cI_2$.
\end{theorem}

Under \Cref{assump:domain}, by \Cref{lem:domain}, we know that the domain of $\phi_{G_i}^s \circ \phi_{G_j}^t(x)$ is exactly $\cI_i(x)\times \cI_j(x)$, thus the above theorem simplifies into the following.

\begin{theorem}\label{thm:commuting_equivalence_with_assumption_domain}
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a $\cC^2$
parametrization satisfying \Cref{assump:domain}.
For any $i, j \in [d]$, $[\nabla G_i, \nabla G_j](x) = 0$ for all $x \in M$ if and only if for any $x \in M$,  it holds that $\phi_{G_i}^s \circ \phi_{G_j}^t(x) = \phi_{G_j}^t \circ \phi_{G_i}^s(x)$ for all $(s,t)\in \cI_1(x) \times \cI_2(x)$.
\end{theorem}

The commuting condition clearly holds when each $G_i$ only depends on a 
different subset of coordinates of $x$, because we then have 
$\nabla ^2G_i (\cdot)\nabla G_j(\cdot)\equiv 0$ for any distinct $i, j \in[d]$ as 
$\nabla^2 G_i$ and $\nabla G_j$ live in different subspaces of $\RR^D$.  
We call such $G$ \emph{separable parametrizations}, and this case covers all the 
previous examples~\citep{gunasekar2018implicit, vaskevicius2019implicit, 
amid2020winnowing, woodworth2020kernel,amid2020reparameterizing}.
Another interesting example is the \emph{quadratic parametrization}: 
We parametrize $w \in \RR^d$ by $G: \RR^D \to \RR^d$ where for each $i \in [d]$, 
there is a symmetric matrix $A_i \in \RR^{D \times D}$ such that 
$G_i(x) = \frac{1}{2} x^\top A_i x$.
Then each Lie bracket $[G_i, G_j](x) = (A_jA_i - A_iA_j)x$, and thus $G$ is a 
commuting parametrization if and only if matrices $\{A_i\}_{i=1}^d$ commute.

For concreteness, we analyze two examples below. 
The first one is both  a separable parametrization and a commuting quadratic 
parametrization. 
The second one is a quadratic parametrization but not commuting.
\begin{example}[$u^{\odot 2}-v^{\odot 2}$ parametrization,~\citealt{woodworth2020kernel}]\label{eg:commuting_param}
Parametrize $w \in \RR^d$ by $w = u^{\odot 2} - v^{\odot 2}$.
Here $D = 2d$, and the parametrization $G$ is given by $G(x) = u^{\odot 2} - v^{\odot 2}$
for $x = \binom{u}{v} \in \RR^D$.    
Since each $G_i(x)$ involves only $u_i$ and $v_i$, $G$ is a separable parametrization 
and hence a commuting parametrization. 
Meanwhile, each $G_i(x)$ is a quadratic form in $x$, and it can be directly 
verified that the matrices underlying these quadratic forms commute with each 
other.   
\end{example}

\newcommand{\xddots}{%
  \raise 4pt \hbox {.}
  \mkern 6mu
  \raise 1pt \hbox {.}
  \mkern 6mu
  \raise -2pt \hbox {.}
}

\begin{example}[Matrix factorization]\label{eg:matrix_factorization}
As a counter-example, consider two parametrizations for matrix factorization: 
$G(U) = UU^\top$ and $G(U,V)=UV^\top$, where $U,V\in\RR^{d\times r}$ and $d\ge 2, r\ge 1$.
These are both \emph{non-commuting} quadratic parametrizations. 
Here we only demonstrate for the parametrization $G(U) = UU^\top$, 
and $G(U,V)=UV^\top$ follows a similar argument.
For each $i, j \in [d]$, we define $E_{ij} \in \RR^d$ as the one-hot matrix with the $(i,j)$-th entry 
being $1$ and the rest being $0$, and denote $\overline E_{ij} = \frac{1}{2} (E_{ij} + E_{ji})$.  
For $r=1$, we have $G_{ij}(U) = U_iU_j = U^\top \overline E_{ij} U$ for any 
$i, j \in [d]$, so $G$ is a quadratic parametrization.
Note that $\overline E_{ii}\overline E_{ij} = \frac{1}{2}E_{ij}
\neq \frac{1}{2}E_{ji} = \overline E_{ij} \overline{E}_{ii}$ for all distinct 
$i,j \in [d]$, which implies that $[\nabla G_{ij}, \nabla G_{ii}] \neq 0$, so $G$ is 
non-commuting.
More generally, we can reshape $U$ as a vector 
$\overrightarrow{U}:= [U_{:1}^\top, \ldots, U_{:r}^\top]^\top \in \RR^{rd}$ 
where each $U_{:j}$ is the $j$-th column of $U$, and 
the resulting quadratic form for the $(i,j)$-entry of $G(U)$ corresponds to a 
block-diagonal matrix:
\begin{align*}
    G_{ij}(U) = (\overrightarrow{U})^\top  \begin{pmatrix}
        \overline{E}_{ij}\\
        &\xddots\\
        &&\overline{E}_{ij}
    \end{pmatrix}\overrightarrow{U}.
\end{align*} 
Therefore, $\nabla^2 G_{ij}$ does not commute with $\nabla^2 G_{ii}$ due to the 
same reason as in the rank-1 case. 
\end{example}

\begin{remark}
This non-commuting issue for general matrix factorization does not conflict with 
the theoretical analysis in \citet{gunasekar2018implicit} where the measurements are 
commuting, or equivalently, only involves diagonal elements, as $\{G_{ii}\}_{i=1}^d$ 
are indeed commuting parametrizations. 
\citet{gunasekar2018implicit} is the first to identify the above non-commuting 
issue and conjectured that the implicit bias result for diagonal measurements 
can be extended to the general case.
\end{remark}

\subsection{Main Equivalence Result}
Next, we proceed to present our analysis for gradient flow with commuting 
parametrization.
The following two lemmas highlight the special properties of commuting parametrizations.
\Cref{lem:gf_commuting} shows that the point reached by gradient flow with any 
commuting parametrization is determined by the integral of the negative gradient 
of the loss along the trajectory.


\begin{lemma}\label{lem:gf_commuting}
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a commuting 
 parametrization.
For any initialization $\xinit \in M$, consider the gradient flow for any 
time-dependent loss $L_\cdot \in \cL$ as in \Cref{def:time_loss}:
\begin{align*}
\diff x(t) =  -\nabla   (L_t \circ G)(x(t)) \diff t, \qquad x(0) = \xinit.
\end{align*}
Further define $\mu(t) = \int_0^t - \nabla L_t(G(x(s))) \diff s$.
Suppose $\mu(t) \in \cU(\xinit)$ for all $t \in [0, T)$ where 
$T \in \RR \cup \{\infty\}$, then it holds that $x(t) = \psi(\xinit; \mu(t))$ 
for all $t \in [0, T)$.
\end{lemma}


Based on \Cref{lem:gf_commuting}, the next key lemma reveals the
essential approach to find the mirror map.


\begin{lemma}\label{lem:commuting_potential}
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a commuting 
and regular parametrization satisfying \Cref{assump:domain}.
Then for any $\xinit \in M$, there exists a Legendre function 
$Q: \RR^d \to \RR\cup\{\infty\}$ such that $\nabla Q(\mu) = G(\psi(\xinit;\mu))$ 
for all $\mu \in \cU(\xinit)$.
Moreover, let $R$ be the convex conjugate of $Q$, then $R$ is also a Legendre 
function and satisfies that $\inter(\dom R) = \Omega_w(\xinit;G)$ and
\begin{align*}
\nabla^2 R(G(\psi(\xinit; \mu))) 
= \big(\partial G(\psi(\xinit; \mu)) \partial G(\psi(\xinit;\mu))^\top\big)^{-1}
\end{align*}
for all $\mu \in \cU(\xinit)$.
\end{lemma}


Next, we present our main result on characterizing any gradient flow with commuting 
parametrization by a mirror flow.


\zhiyuan{change to $L_t$}

\begin{theorem}\label{thm:commuting_to_mirror}
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a commuting 
and regular parametrization satisfying \Cref{assump:domain}.
For any initialization $\xinit \in M$, consider the gradient flow for any 
$\cC^1$ loss function $L:\RR^d\to\RR$:
\begin{align*}
    \diff x(t) = - \nabla (L \circ G)(x(t)) \diff t, \qquad x(0)=\xinit.
\end{align*}
Define $w(t) = G(x(t))$ for all $ t\geq 0$, then the dynamics of $w(t)$ is a 
mirror flow with respect to the Legendre function $R$ given by 
\Cref{lem:commuting_potential}, i.e., 
\begin{align*}
    \diff \nabla R(w(t)) = - \nabla L(w(t))\diff t, \qquad w(0) = G(\xinit).
\end{align*}
Moreover, this $R$ only depends on the initialization $\xinit$ and 
the parametrization $G$, and is independent of the loss function $L$.
\end{theorem}


\begin{proof}[Proof of \Cref{thm:commuting_to_mirror}]
Recall that the gradient flow in the $x$-space governed by $-\nabla (L \circ G)(x)$ is
\begin{align*}
    \diff x(t) = - \nabla (L \circ G)(x(t)) \diff t
    = - \partial G(x(t))^\top \nabla L(G(x(t))) \diff t.
\end{align*}
Using $w(t) = G(x(t))$, the corresponing dynamics in the $w$-space 
is
\begin{align}\label{eq:w_dynamics}
\diff w(t) &= \partial G(x(t)) \diff x(t)
= - \partial G(x(t)) \partial G(x(t))^\top \nabla L(w(t)) \diff t.
\end{align}

By \Cref{lem:gf_commuting}, we know that the solution to the gradient flow 
satisfies $x(t) = \psi(\xinit; \mu(t))$ where $\mu(t) = \int_0^t - \nabla L(G(x(s)))
\diff s$.
Therefore, applying \Cref{lem:commuting_potential}, we get a Legendre function 
$R: \RR^d \to \RR \cup \{\infty\}$ with domain $\Omega_w(\xinit;G)$ such that
\begin{align*}
\nabla^2 R(w(t)) &= \nabla^2 R(G(\psi(\xinit;\mu(t)))) 
= \big(\partial G(\psi(\xinit;\mu(t))) \partial G(\psi(\xinit;\mu(t)))\big)^{-1}
\end{align*}
for all $t\geq 0$.
Then the dynamics of $w(t)$ in \eqref{eq:w_dynamics} can be rewritten as  
\begin{align*}
    \diff w(t) = - \nabla^2 R(w(t))^{-1} \nabla L(w(t)) \diff t,
\end{align*}
or equivalently,
\begin{align*}
    \diff \nabla R(w(t)) = - \nabla L(w(t)) \diff t,
\end{align*}
which is exactly the mirror flow with respect to $R$ initialized at 
$w(0) = G(\xinit)$.
Further note that the result of Lemma~\ref{lem:commuting_potential} is completely 
independent of the loss function $L$, and thus $R$ only depends on 
the initialization $\xinit$ and the parametrization $G$.
This finishes the proof.
\end{proof}

\Cref{thm:commuting_to_mirror} provides a sufficient condition for when a 
gradient flow with certain parametrization $G$ is simulating a mirror flow.
The next question is then: What are the necessary conditions on the parametrization 
$G$ so that it enables the gradient flow to simulate a mirror flow?
We provide a (partial) characterization of such $G$ in the following theorem.

\begin{theorem}[Necessary condition on smooth parametrization to be commuting]
\label{thm:necessary_condition} 
Let $M$ be a smooth submanifold of $\RR^D$ and $G: M \to \RR^d$ be a 
smooth parametrization. 
If for any $\xinit \in M$, there is a Legendre function $R$  such 
that for all time-dependent loss $L_t \in \cL$, the gradient flow under 
$L_t \circ G$ initialized at $\xinit$ can be written as the mirror flow 
under $L_t$ with respect to $R$, then $G$ must be a regular 
parametrization, and it also holds that for each $x\in M$,
\begin{align}\label{eq:necessary_condition}
	\mathrm{Lie}^{\ge 2}(\partial G)\big\vert_{x} \subseteq \mathrm{ker}(\partial G(x)),
\end{align}
where $\mathrm{Lie}^{\ge K}(\partial G):=
\mathrm{span}\big\{[[[[ \nabla G_{j_{1}}, \nabla G_{j_2}], \ldots],
\nabla G_{j_{k-1}}],\nabla G_{j_k}] \mid k\geq K, \forall i \in [k], j_i\in [d]\}$ 
is the subset of the Lie algebra generated by the gradients of coordinate functions 
of $G$ only containing elements of order higher than $K$, and $\mathrm{ker}(\partial G(x))$ is the orthogonal complement of 
$\mathrm{span}(\{\nabla G_i(x)\}_{i=1}^d)$.
\end{theorem}

Note the necessary condition in \eqref{eq:necessary_condition} is weaker than 
assuming that G is a commuting parametrization, and we conjecture that it is indeed sufficient. 
\begin{conjecture}
The claim in \Cref{thm:commuting_to_mirror} still holds, if we relax the 
commuting assumption to that 
$\mathrm{Lie}^{\ge 2}(\partial G)\big\vert_{x} \subseteq \mathrm{ker}(\partial G(x))$ 
for all $x\in M$.
\end{conjecture}

With the above necessary condition in \Cref{eq:necessary_condition}, we can formally refute the possibility that 
one can use mirror flow to characterize the implicit bias of gradient flow for 
matrix factorization in general settings, as summarized in 
\Cref{clrl:matrix_factorization_non_commuting}. 
It is also worth mentioning that \citet{li2019towards} constructed a concrete counter 
example showing that the implicit bias for commuting measurements, 
that gradient flow finds the solution with minimal nuclear norm, does not hold 
for the general case, where gradient flow could prefer the solution with minimal 
rank instead.

\begin{corollary}[Gradient flow for matrix factorization cannot be written as mirror flow]
\label{clrl:matrix_factorization_non_commuting}
For any $d, r \in \NN$, let $M$ be an open set in $\RR^{d\times r}$ and 
$G: M \to \RR^{d\times d}$ be a smooth parametrization given by $G(U) = UU^\top$. 
Then there exists a initial point $\xinit\in M$ and a time-dependent loss $L_t$ 
such that the gradient flow under $L_t\circ G$ starting from $U_{\textrm{init}}$ 
cannot be written as a mirror flow with respect to any mirror map $R$ under 
the loss $L_t$.
\end{corollary}

\begin{proof}[Proof of \Cref{clrl:matrix_factorization_non_commuting}]
It turns out that the necessary condition in \Cref{thm:necessary_condition} is 
already violated  by only considering the Lie algebra spanned by $\{\nabla G_{11},\nabla G_{12}\}$. 
We follow the notation in \Cref{eg:matrix_factorization} to define each
$E_{ij} \in \RR^d$ as the one-hot matrix with the $(i,j)$-th entry being $1$, 
and denote $\overline E_{ij} = \frac{1}{2} (E_{ij} + E_{ji})$ and 
$\Delta_{ij} =E_{ij} - E_{ji}$. 
Then $[\nabla G_{11}, \nabla G_{12}](U) = 4(\overline E_{11}\overline E_{12} - \overline E_{12}\overline E_{11}) U= \Delta_{12}U$ 
and $[\nabla G_{11}, [\nabla G_{11}, \nabla G_{12}]] (U) = ( \overline E_{11}\Delta_{12} - \Delta_{12}\overline E_{11})U = \overline{E}_{12}U$.  Further noting that $\inner{[\nabla G_{11}, [\nabla G_{11}, \nabla G_{12}]]}{ \nabla G_{12}} = 2 \norm{\overline{E}_{12}U}_F^2 = \frac{1}{2}\sum_{i=1}^r (U_{1i}^2 + U_{2i}^2)$ must be positive at some $U$ in every open set $M$, 
by \Cref{thm:necessary_condition}, we know such $U_{\textrm{init}}$ and $L_t$ exist. 
Moreover, $L_t$ will only depend on $G_{11}(U)$ and $G_{12}(U)$.
\end{proof}

The following corollary shows that gradient flow with non-commuting parametrization 
cannot be mirror flow, when the dimension of the reachable set matches with that of the $w$-space.

\begin{corollary}
\label{cor:non_commuting}
Let $M$ be a smooth submanifold of $\RR^D$ whose dimension is at least $d$. 
Let $G: M \to \RR^d$ be a regular parametrization such that for any 
$\xinit \in M$, the following holds:
\begin{enumerate}
    \item[(a)] $\Omega_x(\xinit; G)$ is a submanifold of dimension $d$.
    \item[(b)] There is a mirror map $R$ such that for any time-dependent loss 
    $L_t \in \cL$, the gradient flow governed by $-\nabla  (L_t \circ G)(x)$ with 
    initialization $\xinit$ can be written as a mirror flow with respect to $R$.
\end{enumerate}
Then $G$ must be a commuting parametrization. 
\end{corollary}

\begin{proof}[Proof of \Cref{cor:non_commuting}]
By the condition (b) and \Cref{thm:necessary_condition}, we know that each 
Lie bracket $[\nabla G_i, \nabla G_j] \in \ker(\partial G)$.
By the condition (a), we know that each Lie bracket 
$[\nabla G_i, \nabla G_j] \in \mathrm{span}\{\nabla G_i\}_{i=1}^d$.
Combining these two facts, we conclude that each $[\nabla G_i, \nabla G_j] \equiv 0$, 
so $G$ is a commuting parametrization.	
\end{proof}

Next, we establish the convergence of $w(t) = G(x(t))$ when $x(t)$ is given by 
some gradient flow with the commuting parametrization $G$.
Here we require that the convex function $R$ given by \Cref{lem:commuting_potential} 
is a Bregman function~(see definition in \Cref{apdx:convex_analysis}).
The proofs of \Cref{thm:convergence_commuting_flow},
\Cref{cor:convergence_commuting_flow_Rd} and 
\Cref{cor:convergence_commuting_quadratic_parametrization} are in \Cref{apdx:CGF_to_MF}.

\begin{theorem}\label{thm:convergence_commuting_flow}
Under the setting of \Cref{thm:commuting_to_mirror}, 
further assume that the loss $L$ is quasi-convex, $\nabla L$ is locally 
Lipschitz and $\argmin\{L(w) \mid w \in \dom R\}$ is non-empty where $R:\RR^d 
\to \RR\cup\{\infty\}$ is the convex function given by \Cref{lem:commuting_potential}.
Suppose $R$ is a Bregman function, then as $t \to \infty$, $w(t)$ 
converges to some $w^*$ such that $\nabla L(w^*)^\top (w - w^*) \geq 0$ for all $w \in \dom R$.
Moreover, if the loss function $L$ is convex, then $w(t)$ converges to a minimizer in 
$\overline{\dom R}$.
\end{theorem}

\begin{corollary}\label{cor:convergence_commuting_flow_Rd}
Under the setting of \Cref{thm:convergence_commuting_flow}, if the reachable set 
in the $w$-space satisfies $\Omega_w(\xinit;G) = \RR^d$, then $R$ is a Bregman function and all the statements in \Cref{thm:convergence_commuting_flow} hold.
\end{corollary}



\begin{theorem}\label{cor:convergence_commuting_quadratic_parametrization}
Under the setting of \Cref{thm:convergence_commuting_flow}, consider the 
commuting quadratic parametrization $G: \RR^D \to \RR^d$ where each 
$G_i(x) = \frac{1}{2} x^\top A_ix$, for symmetric matrices 
$A_1, A_2, \ldots, A_d\in\mathbb{R}^{D\times D}$ that commute with each other, 
\emph{i.e.}, $A_iA_j-A_jA_i=0$ for all $i,j\in[d]$. 
For any $\xinit \in \RR^D$, if 
$\{\nabla G_i(\xinit)\}_{i=1}^d = \{ A_i \xinit\}_{i=1}^d$ are linearly independent, 
then the following holds:
\begin{enumerate}
\item[(a)] For all $\mu \in \RR^d$, $\psi(\xinit;\mu ) = \exp(\sum_{i=1}^d \mu_i A_i) \xinit$ where $\exp(\cdot)$ 
is the matrix exponential defined as $\exp(A):= \sum_{k=0}^\infty \frac{A^k}{k!}$.
    
\item[(b)] For each $j \in [d]$ and all $\mu \in \RR^d$, 
$G_j(\psi(\xinit;\mu)) = \frac{1}{2} \xinit^\top \exp(\sum_{i=1}^d 2\mu_i A_i) 
A_j \xinit$.
    
\item[(c)] $Q(\mu) = \frac{1}{4}\norm{\psi(\xinit;\mu)}_2^2 = \frac{1}{4} 
\big\|\exp(\sum_{i=1}^d \mu_i A_i) \xinit\big\|_2^2$ is a mirror map with domain $\RR^d$.
    
\item[(d)] $R$ is a Bregman function with $\dom R = \overline{\range \nabla Q}$ where 
$\range \nabla Q$ is the range of $\nabla Q$, and 
thus all the statements in \Cref{thm:convergence_commuting_flow} hold.
\end{enumerate}
\end{theorem}


\subsection{Solving underdetermined linear regression with commuting parametrization}
Next, we specialize to underdetermined linear regression problems to 
showcase our framework.

\paragraph{Setting: underdetermined linear regression.}
Let $\{(z_i,y_i)\}_{i=1}^n \subset \RR^d \times \RR$ be a dataset of size $n$. 
Given any parametrization $G$, the output of the linear model on the $i$-th data is $z_i^\top G(x)$.
The goal is to solve the regression for the label vector $Y = (y_1, y_2, \ldots, y_n)^\top$.
For notational convenience, we define $Z = (z_1, z_2, \ldots, z_n) \in \RR^{d \times n}$. 

We can apply \Cref{thm:mf_implicit_bias} to obtain the implicit bias of gradient
flow with any commuting parametrization.
\begin{theorem}\label{thm:bias_linear_model}
Let $M$ be a smooth submanifold of $\RR^d$ and $G: M \to \RR^d$ be a commuting 
and regular parametrization satisfying \Cref{assump:domain}.
Suppose the loss function $L$ satisfies $L(w) = \widetilde L(Zw)$ for some 
differentiable $\widetilde L: \RR^n \to \RR$.
For any $\xinit \in M$, consider the gradient flow 
\begin{align*}
    \diff x(t) = -\nabla (L \circ G)(x(t)) \diff t, \qquad x(0) = \xinit.
\end{align*}
There exists a convex function $R$  
(given by \Cref{lem:commuting_potential}, depending only on the initialization 
$\xinit$ and the parametrization $G$), such that for any dataset 
$\{(z_i, y_i)\}_{i=1}^n \subset \RR^d \times \RR$, if $w(t) = G(x(t))$ converges 
as $t \to \infty$ and the convergence point $w_\infty = \lim_{t \to \infty} w(t)$ 
satisfies $Z w_\infty = Y$, then 
\begin{align*}
    R(w_\infty) = \min_{w: Zw=Y} R(w),
\end{align*}
that is, gradient flow implicitly minimizes the convex regularizer $R$ among all
interpolating solutions.
\end{theorem}

\begin{proof}[Proof of \Cref{thm:bias_linear_model}]
By \Cref{thm:commuting_to_mirror}, $w(t)$ obeys the following mirror flow:
\begin{align*}
    \diff \nabla R(w(t)) = -\nabla L(w(t)) \diff t,\qquad w(0) = G(\xinit).
\end{align*}
Applying \Cref{thm:mf_implicit_bias} yields 
\begin{align*}
    D_R(w_\infty, G(\xinit)) = \min_{w: Zw=Y} D_R(w, G(\xinit)).
\end{align*}
Therefore, for any $w \in \inter(\dom R)$ such that $Zw = Y$, we have 
\begin{align*}
    &R(w_\infty) - R(G(\xinit)) - \langle \nabla R(G(\xinit), w_\infty - G(\xinit)\rangle\\
    &\qquad \leq R(w) - R(G(\xinit)) - \langle \nabla R(G(\xinit), w - G(\xinit)\rangle
\end{align*}
which can be reorganized as 
\begin{align}\label{eq:convergence_point}
    R(w_\infty) \leq R(w) - \langle \nabla R(G(\xinit)), w - w_\infty\rangle.
\end{align}
Note that by \Cref{lem:commuting_potential}, we also have 
\begin{align}\label{eq:R_property}
    \nabla R(G(\xinit)) = \nabla R(G(\psi(\xinit; 0))) = \nabla R(\nabla Q(0)) = 0
\end{align} 
where the last equality follows from the property of convex conjugate.
Combining \eqref{eq:convergence_point} and \eqref{eq:R_property}, we get 
$R(w_\infty) \leq R(w)$ for all $w \in \inter(\dom R)$ such that $Zw = Y$.
By the continuity of $R$, this property can be further extended to the entire
$\dom R$, and for any $w \notin \dom R$, we have $R(w) = \infty$ by definition, 
so $R(w_\infty) \leq R(w)$ holds trivially.
This finishes the proof.
\end{proof}

Note that the identity parametrization $w = G(x) = x$ is a commuting parametrization. 
Therefore, if we run the ordinary gradient flow on $w$ itself and it converges 
to some interpolating solution, then the convergence point is closest to the 
initialization in Euclidean distance among all interpolating solutions.
This recovers the well-known implicit bias of gradient flow for underdetermined 
regression.

Furthermore, we can recover the results on the quadratically overparametrized 
linear model studied in a series of papers~\citep{gunasekar2018implicit,woodworth2020kernel,azulay2021implicit},
as summarized in the following \Cref{cor:overparam_linear_model}.
Note that their results assumed convergence in order to characterize the 
implicit bias, whereas our framework enables us to directly prove the 
convergence as in \Cref{cor:convergence_commuting_quadratic_parametrization}, 
where the convergence guarantee is also more general 
than existing convergence results for \Cref{eg:commuting_param} 
in~\citet{pesme2021implicit,li2022what}.

\begin{corollary}\label{cor:overparam_linear_model}
Consider the underdetermined linear regression problem with data $Z \in \RR^{d \times n}$
and $Y \in \RR^n$.
Let $\widetilde{L}: \RR^n \to \RR$ be a differentiable loss function such that 
$\widetilde L$ is quasi-convex, $\nabla \widetilde{L}$ is locally Lipschitz, 
and $Y \in \RR^n$ is its unique global minimizer. 
Consider solving $\min_{w}\widetilde{L}(Zw)$ 
by running gradient flow on $L(w) = \widetilde L(Zw)$ with the quadratic 
parametrization $w = G(x) = u^{\odot 2} - v^{\odot 2}$ where 
$x = \binom{u}{v} \in \RR^{2d}_+$, for any initialization $\xinit \in \RR^{2d}_+$:
\begin{align*}
    \diff x(t) = - \nabla (L \circ G)(x(t)) \diff t, 
    \qquad x(0) = \xinit.
\end{align*}
Then as $t \to \infty$, $w(t) = G(x(t))$ converges to some $w_\infty$ such that 
$Zw_\infty = Y$ and 
\begin{align*}
    R(w_\infty) = \min_{w: Zw = Y} R(w)
\end{align*} 
where $R$ is given by
\begin{align*}
R(w) = \frac{1}{4} \sum_{i=1}^d \Big(w_i \arcsinh \Big(\frac{w_i}{2u_{0,i} v_{0,i}}\Big) 
- \sqrt{w_i^2 + 4 u^2_{0,i} v^2_{0,i}} - w_i\ln \frac{u_{0,i}}{v_{0,i}}\Big).
\end{align*}
\end{corollary}



\section{Every mirror flow is a gradient flow with commuting parametrization}\label{sec:MF_to_CGF}
Consider any smooth Legendre function $R: \RR^d \to \RR\cup\{\infty\}$, and 
recall the corresponding mirror flow:
\begin{align*}
    \diff \nabla R(w(t)) &= - \nabla L(w(t)) \diff t.
\end{align*}
Note that $\inter(\dom R)$ is a convex open set of $\RR^d$, hence a smooth 
manifold (see Example 1.26 in~\citet{lee2013smooth}).
Then $\nabla^2 R$ is a continuous positive-definite metric on $\inter(\dom R)$.
As discussed previously, the above mirror flow can be further rewritten as the 
Riemannian gradient flow on the Riemannian manifold $(\inter(\dom R), \nabla^2 R)$, 
\emph{i.e.}, 
\begin{align*}
    \diff w(t) = -\nabla^2 R(w(t))^{-1} \nabla L(w(t)) \diff t.
\end{align*}
The goal is to find a parametrization $G: U \to \RR^d$, where $U$ is 
an open set of $\RR^D$ and initialization $\xinit \in U$, such that the dynamics 
of $w(t) = G(x(t))$ can be induced by the gradient flow on $x(t)$ governed 
by $-\nabla (L \circ G)(x)$. 
Formally, we have the following result:

\begin{theorem}\label{thm:mirror_to_commuting}
Let $R: \RR^d \to \RR \cup \{\infty\}$ be a smooth Legendre function. 
There exist a smooth and regular submanifold of $\RR^D$ denoted by $M$, an open neighborhood 
$U$ of $M$ and a parametrization $G: U \to \RR^d$ such that for any mirror flow 
on any $\mathcal{C}^1$ loss function $L$ with any initialization $\winit \in 
\inter(\dom R)$
\begin{align}\label{eq:mirror_flow_init}
    \diff \nabla R(w(t)) = - \nabla L(w(t)) \diff t, \quad w(0)=\winit,
\end{align}
it holds that $w(t) = G(x(t))$ for all $t \geq 0$ where $x(t)$ is given by the 
gradient flow under the objective $(L \circ G)$ initialized at $\xinit$, i.e., 
\begin{align}\label{eq:gradient_flow_init}
    \diff x(t) = - \nabla (L \circ G)(x(t)) \diff t, \quad x(0)=\xinit.
\end{align}
Moreover, $G$ restricted on $M$, denoted by $G\vert_M$ is a commuting and regular parametrization 
and $\partial G = \partial G\vert_M$ on $M$, which implies $x(t)\in M$
for all $t\ge 0$. 
If $R$ is further a mirror map, then $\{\nabla G_i|_M\}_{i=1}^d$ are complete 
vector fields on $M$. 
\end{theorem}

To illustrate the idea, let us first suppose such a smooth and regular 
parametrization $G$ exists and is a bijection between the reachable set $\Omega_x(\xinit;G)\subset \RR^D$ and $\inter(\dom R)$, 
whose inverse is denoted by $F$. 
It turns out that we can show
\begin{align*}
\partial F(w)^\top \partial F(w) 
= (\partial G(F(w)) \partial G(F(w))^\top)^{-1}
= \nabla^2 R(w)
\end{align*} 
where the second equality follows from the relationship between $R$ and $G$ as discussed in the introduction on~\Cref{eq:gf_w}.
Note that this corresponds to expressing the metric tensor $\nabla^2 R$ using an 
explicit map $F$, which is further equivalent to embedding the Riemannian 
manifold $(\inter(\dom R), \nabla^2 R)$ into a Euclidean space $(\RR^D,\overline{g})$ in a way 
that preserves its metric.
This refers to a notion called isometric embedding in differential geometry.

\begin{definition}[Isometric embedding]\label{defi:isometric_embedding}
Let $(M, g)$ be a Riemannian submanifold of $\RR^d$.
An \emph{isometric embedding} from $(M, g)$ to  $(\RR^D,\overline{g})$ is an differentiable injective map
$F: M \to \RR^D$ that preserves the metric in the sense that for any two tangent vectors $v, w \in T_x(M)$ we have 
$g_x(v, w) = \overline{g}_x(\partial F(x) v, \partial F(x) w)$ where the standard euclidean metric tensor $\overline{g}$ is defined as $\overline{g}_x(u,v) = \inner{u}{v}$ for all $u,v\in\RR^d$.
\end{definition}

Nash's embedding theorem is a classic result in differential geometry that 
guarantees the existence of isometric embedding of any Riemannian manifold into 
a Euclidean space with a plain geometry. 
\begin{theorem}[Nash's embedding theorem, \citealt{nash1956imbedding,gunther1991isometric}]
\label{thm:isometric_embedding}
Any $d$-dimensional Riemannian manifold has an isometric embedding to $(\RR^D,\overline{g})$ 
for some $D\geq d$.
\end{theorem}

The other way to understand \Cref{thm:commuting_to_mirror} is that we can view $\nabla^2 R(w)^{-1} \nabla L(w)$ as the gradient of $L$ with respect to metric tensor $g_R$, where $g^R$ is the Hessian metric induced by strictly convex function $R$ in the sense $g^R_x(u,v):= u^\top\nabla^2 R(x)v$ for any $u,v\in\RR^d$. It is well-known that gradient flow is invariant under isometric embedding and thus we can use Nash's embedding theorem to write the gradient flow on riemmanian manifold $(\inter(\dom R), g^R)$ as that on $(\RR^D, \overline{g})$.
